BriskStream: Scaling Data Stream Processing on Shared-Memory Multicore Architectures

We introduce BriskStream, an in-memory data stream processing system (DSPSs) specifically designed for modern shared-memory multicore architectures. BriskStream's key contribution is an execution plan optimization paradigm, namely RLAS, which takes relative-location (i.e., NUMA distance) of each pair of producer-consumer operators into consideration. We propose a branch and bound based approach with three heuristics to resolve the resulting nontrivial optimization problem. The experimental evaluations demonstrate that BriskStream yields much higher throughput and better scalability than existing DSPSs on multi-core architectures when processing different types of workloads.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> algorithms.tex <==
\section{Optimization Algorithms}
\label{sec:algo}
In this section, we first analyze the resource constraints that the algorithm needs to be aware of (Section~\ref{subsec:constraint}).
Then, we discuss the complexity of the ``naive" searching algorithm for the optimal execution plan (Section~\ref{subsec:complexity}), followed by the improved algorithms including placement algorithm (Section~\ref{subsec:placement}) to determine the optimal operator placement assuming operator replication level is fixed and scaling algorithm (Section~\ref{subsec:parallelism}) that work with the placement algorithm by considering varying operator replication to finally determine the optimal execution plans.

\subsection{Resource Constraints}
\label{subsec:constraint}
We consider three kinds of resource constraints and the optimization algorithm tries to make sure the execution plans satisfy those constraints. 
Task oversubscribing has been studied in some earlier work~\cite{5470434}, but it is not the focus of this paper.
%we don't consider task oversubscribing

\begin{myitemize}
%  %\vspace{-5pt}
    \item \emph{CPU capacity.} 
    Given the available CPU cycles in a CPU socket $S_i$ as \saven{$\epsilon*\kappa$} per unit of time, where $\epsilon$ is the cycles available of single CPU core, and $\kappa$ is the number of CPU cores on a socket. 
    % Denote $\vec{Prod(c)}$ as a set of producers of operator $O_c$.
    The aggregated demand of CPU cycle per unit of time requested from operators, which are scheduled to CPU socket $S_i$ must be smaller than $\epsilon*\kappa$, i.e., 
     %\vspace{-5pt}
    \begin{align} 
        \scriptsize
        &\sum_{c=1}^{m}\sum_{s\in \vec{Prod(c)}}p_{c,i}*{\overline{\mu}}_{s,c}*\xi_{s,c}\leq \epsilon*\kappa\nonumber\\
        &where\     p_{c,i} \in {0,1}, \forall c \in {1,..,m},\forall i \in {1,..,n} \nonumber\\
        &p_{c,i} =1\ \text{if $O_c$ is allocated into $S_i$}
        \label{eqn:amountC}
    \end{align}
     %\vspace{-10pt}
    \item  \emph{Local memory bandwidth capacity.}
    Given the maximum attainable local DRAM bandwidth as $B_i$ per unit of time on socket $S_i$.
    The aggregated amount of bandwidth requested to the same CPU socket $S_i$ per unit of time must be smaller than $B_i$, i.e.,
     %\vspace{-5pt}
    \begin{align} 
         \scriptsize
        &\sum_{c=1}^{m}\sum_{s\in \vec{Prod(c)}}p_{c,i}*{\overline{\mu}}_{s,c}*|M|\leq B_i \nonumber\\
        &where\
        |M| =|Miss_{LLC}|*|cacheLine|\nonumber\\
        &p_{c,i} \in {0,1}, \forall c \in {1,..,m},\forall i \in {1,..,n}\nonumber\\
        &p_{c,i}=1\ \text{if $O_c$ is allocated into $S_i$}
        \label{eqn:constraint_m}
    \end{align}  
     %\vspace{-10pt}
    \item  \emph{\saven{Remote channel bandwidth capacity}.} 
    Given the maximum attainable remote channel bandwidth from socket $S_i$ to $S_j$ as $Q_{i,j}$ bytes per unit of time. 
    The aggregated data transfer from socket $S_i$ to socket $S_j$ per unit of time must be smaller than $Q_{i,j}$, i.e.,
     %\vspace{-5pt}
    \begin{align} 
        \scriptsize
        &\sum_{c=1}^{m}\sum_{s\in \vec{Prod(c)}}p_{c,j}*p_{s,i}*{r}_{s,c}*|tuple|\leq Q_{i,j}\nonumber\\
        &where\ p_{k,i} \in {0,1}, \forall k \in {1,..,m},, \forall i,j \in {1,..,n} \nonumber\\
        &p_{k,i} =1\ \text{if $O_k$ is allocated into $S_i$}
        \label{eqn:constraint_q}
    \end{align}
% %\vspace{-10pt}
\end{myitemize}

\subsection{Complexity Analysis}
\label{subsec:complexity}
Naively, RLAS concerns the scheduling decisions (i.e., $\binom{m}{1}$, where $m$ is the number of CPU sockets) for all $n$ operators. 
Furthermore, as we need to consider different replication configurations for each operator, and assume replication of each operator can be set from $1$ to $K$, we have to consider in total $K^{n}$ different replication configurations.
As a result, the solution space of the presented problem has a size of $O(m^n*K^{n})$, which makes brute-force unpractical for large DAGs (i.e., $n$ is large).

\subsection{Placement Algorithm}
\label{subsec:placement}
Due to resource constraints, the placement \saven{decisions are sometimes conflicting each other} and ordering constraint is introduced into the problem. 
For instance, scheduling of an operator into a socket may prohibit some other operators to be scheduled to the same socket. 
This makes the sub-problem dependent on each other and classical approaches like dynamic programming not suitable.
On the other hand, Branch and Bound (B\&B) are successfully applied in many works~\cite{MORRISON201679} in dueling with non-convex combinatorial optimization problems. 
In this section, we discuss our B\&B based algorithm to solve the RLAS problem assuming operator replication is given and fixed.
    
\textbf{Algorithm overview.}
Branch and Bound (B\&B) systematically enumerates a tree of candidate solutions, based on a bounding function. 
We first define three types of nodes in the tree: the solution nodes, the live nodes, and the dead nodes. 

\emph{Live nodes:} 
the live node contains the solution that violates some constraints and they can be expanded into other nodes that violate fewer constraints. 

\emph{Dead node:} 
once expanded, a live node is turned into a dead node, and we do not have to remember it anymore. 

\emph{Solution node:} 
solution node contains a scheduling plan without violating any constraint. 
The value of a solution node comes directly from the performance model. 
The algorithm may reach multiple solution nodes as it explores the solution space. 
The solution node with the best value is the output of the algorithm. 

Before presenting our algorithm based on B\&B, we need to first determine three main components of this algorithm, 
1) the bounding function so that the algorithm can efficiently estimate the bounded cost of the live solution,
2) a strategy for selecting the live solution to be investigated in the current iteration,
and 3) a branching rule to be applied if the live solution needs to be further explored.
    
\textbf{The bounding function.}
If the bounding function value of an intermediate node is worse than the best feasible solution obtained so far, we can safely prune it and all of its children nodes. 
This does not affect the optimality of the algorithm because the value of a live node must be better than all its children node after further exploration. 
In other words, the value of a live node is the theoretical upper bound of the subtree of nodes.

\tony{The bounded problem that we used in our optimizer originates from the same optimization problem with relaxed constraints that every non-scheduled operator can be scheduled in order to maximize its process rate. 
Specifically, the value (objective function) of every intermediate solution is obtained by fixing the allocation of 
\emph{valid} operators and maximizing processing rates of every non-scheduled ones.
}

\begin{algorithm}[t]
    \scriptsize
    \caption{Branch and Bound based Placement}\label{alg:algo}
    \begin{algorithmic}[1]
        \DATA Stake: $stack$;\Comment{contains all live nodes}
        \DATA Node: $solution$;
        \DATA Node: $e$;\Comment{the current visiting node}
        \RESULTS Scheduling plan: $p$;
        %        \If{apply TSS Algorithm to get an initial solution}
        %        \State $solution.plan$ $\leftarrow$ $TSS()$
        %        \Else
        \State $solution.value$ $\leftarrow$ $0$\Comment{Start with no initial solution}
        %        \EndIf
        \newline /*Initialize the root node*/
        \State $e.decisions$  $\leftarrow$ a list contains all possible collocation decisions;
        \State $e.plan$ $\leftarrow$ all operators are collocated into the same CPU socket;
        \State $e.validOperators$ $\leftarrow$ 0;
        \State Push($stack$,$e$); 
        \newline /*Branch and Bound process*/
        \While {$\neg$IsEmpty($stack$)}
        \State $e$ $\leftarrow$ Pop($stack$);
        \If {$e.validOperators$ = totalOperators} 
        \If {$e.value \geq solution.value$}
        \State $solution$ $\leftarrow$ $e$;
        \EndIf
        \ElsIf{$e.value>solution.value$}
        \State \emph{Branching}($e$);
        \EndIf
        \EndWhile
        \State \Return solution;
        \phase{Branching(Node $e$)}
        \DATA Node[] $children$ $\leftarrow$  \emph{ChildrenOf}($e$);
        %        \ForEach {Node c \in $children$}
        %        \State    c.validOperators  $\leftarrow$ e.validOperators + $\#newAllocatedOperators$;
        %        \State    c.value $\leftarrow$ BoundValue(c);
        %        \EndFor
        \ForEach {Node c $\in$ $children$}
        \State c.validOperators $\leftarrow$ e.validOperators + $\#newAllocate$;
        \State c.value $\leftarrow$ CostFunction(c);
        \EndFor
        \State SortByValue($children$);\Comment{for best first search}
        \State PushAll($stack$,$children$);
        \phase{ChildrenOf(Node $e$)}
        \DATA Node[] $children$;
        \ForEach {pair of $O_s$ and $O_c$ in $e.decisions$}        
        \If{all predecessors are determined except $O_s$ to $O_c$}                
        \newline \*As the process rate can be determined in this case, we apply best fit first strategy for each case.*/    
        \State create nodes of 1): collocating them and 2): separately allocate them; 
        \State add both nodes to $children$;                     
        \Else{}
        \ForEach {way of scheduling $O_s$ and $O_c$}
        \State add one node to $children$;
        \EndFor
        \EndIf
        \EndFor    
        \State \Return $children$;
    \end{algorithmic}
\end{algorithm}


\begin{example}
\label{example2}
Consider the same application in previous example with operators A, A' and B as shown in Figure~\ref{fig:estimate_example2}.
Assume at one iteration, A and A' are scheduled to socket 0 and 1, respectively (i.e., they become valid). 
We are to calculate the bounding function value assuming B is the sink operator, which awaits to be allocated.

In order to calculate the bounding function value, we can simply try to maximize process rates of B. 
In this case, we set B to be collocated with A and A' at the same time (which is certainly invalid), and its out rate is maximized, which is the bounding value of the current iteration.

\begin{figure}
    \centering
    \includegraphics*[width=0.3\textwidth]{example2}
    \caption{Estimating bounding value.}                   
    \label{fig:estimate_example2}
        %\vspace{-10pt}
\end{figure}
\end{example}

\textbf{The searching strategy.}
We adopt a combination strategy of depth first search (DFS) and best first search (BeFS). 
In particular, the basic searching strategy follows DFS, but we always try first the node with a better bounded value between nodes at the same level of the search tree.
This heuristic will not reduce the solution space, but instead, gives a greedy direction on which intermediate node to visit first. The worst case is that all solutions need to be explored. Nevertheless, our experimental results show that this searching heuristic helps in converging towards the best solution faster.
    
\textbf{The branching rule.} 
Naively in each iteration, there are  $\binom{n}{1}*\binom{m}{1}=n*m$ possible solutions to branch (i.e., schedule which operator to which socket) and an average $n$ depth (i.e., one operator is allocated in each iteration). 
In other words, it will still need to examine on \emph{average} $(n*m)^{n}$ candidate solutions~\cite{Devroye:1999:CBB:329857.329859}.
In order to further reduce the complexity of the problem, heuristics have to be applied.
The branching rule determines the generation of children nodes of each live node if it needs to be further explored.
We introduce two heuristics that work together to significantly reduce the solution space as follows.
    
\emph{Collocation heuristic:}
Naively, we need to consider branching to all scheduling decisions of each operator in each iteration. 
However, we observe that some scheduling decisions have \emph{no or little} impact on the process rate of any operators. 
%It turns out that during each iteration, we should at least consider the decisions that involve a pair of producer and consumer together. 
Therefore, we propose to consider a list of collocation decisions instead of scheduling decisions of each operator. During process, we can remove those collocation decisions from list that are no longer relevant. 
For instance, it can be safely discarded (i.e., do not need to consider anymore) if both producer and consumer in the collocation decision are already allocated.
    
%In most cases, the branching heuristics dramatically reduces both the number of possible branches in each iteration and the depth (i.e., two, instead of one, operators may be allocated in one iteration). 
%Hence, it significantly improves the efficiency of searching.
    
\emph{Best-fit heuristic:}
Consider each collocation decision involving a pair of producer and consumer, when all predecessors (i.e., upstream operators) of them are already scheduled, the process rate of them can be determined.
In this case, we select the best-possible plan among them with \emph{best fit} strategy.
Specifically, if two operators can be {collocated} into different sockets, we only consider the way of collocating them into one socket that will leave with the smallest idle resource. 
%Otherwise, if they cannot be collocated, we schedule producer followed by consumer and we consider the way of best fit when multiple sockets can be used.
%On the other hand, when any predecessor is not yet scheduled, we may have to branch to all possible allocation combinations (i.e., $m^2$) due to the undetermined process rate~\footnote{This is often not necessary as we can avoid repeat branching to those identical sockets.}. 

\textbf{Algorithm implementation.}
Algorithm~\ref{alg:algo} illustrates the \emph{Branch and Bound based Placement} algorithm. 
Initially, no valid solution has been found so far and the best objective value is $0$ (i.e., zero output rate)~\footnote{BriskStream applies a fast greedy approach to obtain a valid solution first to speed up the searching process.}. 
The algorithm proceeds with this and it updates the best solution whenever a feasible solution is found. 
The searching process dynamically generates a search tree, which initially only contains the root. 
The root contains the scheduling plan of all operators being collocated and has the upper bound value of the whole solution space. 
During iteration, scheduling decisions are made which update the list of children node  (i.e., branches) by removing those decisions involving producer and consumer have been already allocated. 
The unexplored subspaces are represented as nodes and each iteration processes one such node.

\begin{example}
As a concrete example to illustrate the algorithm, consider scheduling the same application in previous example with an additional operator C as a consumer of B to a machine with two CPU sockets as shown in the top-left of Figure~\ref{fig:algorithm}. Both operator B and C are sink operators. 
\tony{In this example, we assume the aggregated resource demands of three operators with either A, B and C or A', B and C exceed resource constraint of a socket, and they cannot be collocated in the same socket due to violation of resource constraints.}
We also show one feasible solution besides, which is assumed to be the optimal allocation in this example.
The bottom left of Figure~\ref{fig:algorithm} shows how our algorithm explores the searching space by expanding nodes, where the label on the edge represents the collocation decision considered in the current iteration. 

\tony{The detailed states of four nodes are illustrated on the right hand side of the figure, where the state of each node is represented by a two-dimensional matrix.}
The first (horizontal) dimension describes a list of collocation decisions, 
while the second one the operators that interests in this decision. 
A value of `-' means that the respective operator is not interested in this collocation decision.
A value of `1' means that the collocation decision is made in this node, although it may violate resource constraints. 
A value of `0' means that the collocation decision is not satisfied and the involved producer and consumer are separately located. 

At root node, we consider a list of scheduling decisions involving each pair of producer and consumer. 
At Node \Csharp{}1, the collocation decision of A and B is going to be satisfied (i.e., all sockets are empty now), and assume they are collocated to socket 0 (S0). 
However, the solution to the bounding function of this node indicates that while we try to maximize output rates of every pipeline, B and C has to be allocated separately because of the assumed resource constraints in this example. 
As a result, its bounding value is worse than the known feasible solution, and we can stop further exploring this node.

On the other hand, consider Node \Csharp{}3, we first try to collocate B and C, which is also satisfied, and similarly assume they are collocated to socket 0 (S0). 
In this simple example, the solution to the bounding function of this node is identical to the feasible solution, and we need to further explore it.

Finally, we should notice the importance of the heuristics. 
Without the collocation heuristic, root node would generate $2*4$ (instead of $3$) different child nodes, where each child node contains a plan of allocating one of the four operators to one of the two socket.

\begin{figure}[t]
    \centering
    \includegraphics[width=.49\textwidth]{algorithm_example}
    \caption{Placement Algorithm at Runtime.}
    \label{fig:algorithm}
    %\vspace{-5pt}
\end{figure}
\end{example}

        
\subsection{Scaling Algorithm}
\label{subsec:parallelism}
An application has different optimal placement plans under different replication configurations. 
Therefore, determining the optimal replication configuration shall be done together with the placement optimization. 

Algorithm~\ref{alg:algo2} illustrates our \emph{iterative scaling} algorithm. 
Initially, we set replication of each operator to be one (Line 1$\sim$2).
The algorithm proceeds with this and it determines the optimal placement based on its current replication setting (Line 6). 
Then, it stores the current setting if it ends up with better performance (Line 7$\sim$9). 
Subsequently, it increases replication level of the identified bottleneck operator (i.e., this is identified during placement optimization), and determines the optimal placement again (Line 13$\sim$ 23).
At Line 13$\sim$14, we iterate over all the sorted list from topologically sorting on the DAG in parallel. 
This ensures that we have gone through all the way of scaling the topology bottlenecks and hence ensures the optimality of our scaling algorithm. 
We set an upper limit on the total replication level (e.g., usually set to the total number of CPU cores) to stop the recursion. 
At Line 10\&20, either the algorithm hits the scaling upper bound or fails to find a feasible plan will cause the searching to terminate.

\begin{algorithm}[t]
    \scriptsize
    \caption{Topologically sorted iterative scaling}\label{alg:algo2}
    \begin{algorithmic}[1]
        \DATA Execution Plan: $c$;\Comment{the current visiting plan}
        \DATA Execution Plan: $opt$;\Comment{the optimal plan}
        \State $c.parallelism$ $\leftarrow$ set parallelism of all operators to be 1;
        \State $c.graph$ $\leftarrow$ creates execution graph according to $c.parallelism$;
        \State $opt.throughput$ $\leftarrow$ 0;
        \State \emph{Searching($c$)};
        \State \Return $opt$;
        \phase{Searching($c$)}
        \State $c.placement$ $\leftarrow$ optimal placement of $c$;
        \If{$c.throughput>opt.throughput$}
        \State $opt$ $\leftarrow$ $c$;
        \Else{
        \If{failed to find feasible placement plan}
        \Return;
        \EndIf
        }
        \EndIf
        \State sorted-lists   $\leftarrow$ Topological\_sort (c.graph)
        \ForEach{list:sorted-lists}
        \ForEach{Executor $e$ $\in$ list}
        \If{$e$ is bottleneck}
        \State $c$ $\leftarrow$ Increase the parallelism of $e$ by 1;
        \EndIf
        \EndFor
        \If{failed to further increase the parallelism}
        \Return;
        \Else
        \State \emph{Searching($c$)};
        \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm}
    
\tony{We set an upper bound of 600 seconds for running RLAS algorithm, which are usually enough to optimize the workload. Otherwise, the best feasible plan obtained is returned as the optimization result.
As the streaming application potentially runs forever, the overhead of generating a plan is not included in our measurement.}

==> design.tex <==
\section{System Overview}
\label{sec:design}
The design goal of Brisk is to support the same APIs of the popular DSP systems (e.g., Storm) while optimizing the system performance as much as possible targeting at shared-memory multicores.

Brisk follows the basic architectures including pipelined and operator replication designs of modern DSP systems as introduced in Section~\ref{sec:background}. 
%Specifically, each operator is treated as a single execution unit (e.g., a Java thread), whose CPU affinity can be configured (i.e., operator placement) and operator can be replicated into multiple copies (i.e., operator replication) running in parallel for higher throughput. 
Such design is well known for its advantage of low processing latency and being adopted by many DSP systems such as Storm~\cite{Storm}, Flink~\cite{flink}, SEEP~\cite{seep}, and Heron~\cite{heron}, but requires fine-grained operator replication and placement optimization.

Due to resource constraint, operator and its producers may not be scheduled into the same CPU sockets. As a result, operator experiences additional remote memory access (RMA) penalty during input tuple fetch. 
A bad execution plan may either oversubscribe a few CPU sockets that induce significant contention overhead or introduces unnecessary RMA communication.
%and a NUMA-aware optimization strategy is needed. 
We propose a fine-grained performance model that takes relative location (i.e., relative NUMA distance to each of its producers) of each operator into consideration, which can accurately predict the execution behavior of the application under different execution plans. 
We propose a branch and bound based algorithm to solve the resulting placement problem under the NUMA effect, and we further design a light-weight approach to identify the final execution plan considering both operator replication and placement configurations. 
%In the following of this paper, we further discuss our execution plan optimization in detail.

==> distribute.tex <==
\section{Multi-NUMA Servers}

==> model.tex <==
\section{Performance Model}
\label{sec:model}
In the following, we discuss our NUMA-aware performance model that guides the optimization.
Our model is inspired by rate-based optimization framework~\cite{Viglas:2002:RQO:564691.564697}, but the original rate-based optimization framework assumes processing capability of an operator is predefined and independent of different execution plans. Moreover, it is neither replication-aware nor NUMA-aware, which are both necessary for our problem. 
%For instance,  processing rate (i.e., how many tuples can be processed in a unit of time) of an operator is modelled to be fixed and 

\textbf{Model overview.}
In this paper, application throughput is the metric to maximized by optimizations.
The throughput ($\Psi$) of the stream application is modelled as the summation of the number of outputs produced in a unit of time (i.e., $r_{operator}$ ) from all ``sink" operators (i.e., operators with no consumer). That is,
\begin{align} 
\scriptsize
    \Psi=\sum_{sink}{r_{sink}}
\end{align}
Subsequently, in order to predict $r_{sink}$, i.e., the output rate of each ``sink" operator, we need to predict how many tuples it can process in a unit of time (i.e., processing rate) and how many tuples it is expected to receive in a unit of time (i.e., input rate) under an execution plan.
We summarize the main terminologies used in Table~\ref{tbl:notations}. 

\begin{table}[]
    \centering
    \caption{Summary of main terminology}
    %\vspace{-3pt}
    \label{tbl:notations}
    \resizebox{0.49\textwidth}{!}{%
        \begin{tabular}{|l|l|l|l|}
            \hline
            \multicolumn{2}{|l|}{Notation}                & Definitions                                                                                                                                                                      & Sources                                                                                                                               \\ \hline
            \multicolumn{2}{|l|}{$\varepsilon$}                & Cycles available per unit of time in one CPU core                                                                                                                                & 
            \multirow{4}{*}{
                \begin{tabular}[c]{@{}l@{}} platform \\ input \end{tabular} 
            }                                                                                                       \\ \cline{1-3}
            \multicolumn{2}{|l|}{$\kappa$}                & Number of CPU cores per socket of the system                                                                                                                                     &                                                                                                                                       \\ \cline{1-3}
            \multicolumn{2}{|l|}{$\eta_{i,j}$}            & \begin{tabular}[c]{@{}l@{}} Data transfer latency from  socket $i$ to socket $j$, $\eta_{i,i}=0$\end{tabular}                                                  &                                                                                                                                       \\ \cline{1-3}
            \multicolumn{2}{|l|}{$S_i$,$i$,$\in$ $1...n$} & Set of CPU sockets of the system                                                                                                                                                 &                                                                                                                                       \\ \hline
            \multicolumn{2}{|l|}{$\chi$}                  & External input stream rate of a stream application                                                                                                                               & \multirow{3}{*}{    \begin{tabular}[c]{@{}l@{}} application \\ input \end{tabular} }                                                                                                    \\ \cline{1-3}
            \multicolumn{2}{|l|}{$O_j$, $j \in 1...m$}    & Set of operators of a stream application                                                                                                                                         &                                                                                                                                       \\ \cline{1-3}
            \multicolumn{2}{|l|}{$\sigma^{in,br,out}$}    & Input, branch, and output selectivity of an operator                                                                                                                                               &                                                                                                                                       \\ \hline
            %                    \multicolumn{4}{|l|}{}
            %            \\ \hline    
            \multicolumn{2}{|l|}{$|tuple| $}                  & average size of each input tuple  of an operator                                                             & \multirow{3}{*}{    \begin{tabular}[c]{@{}l@{}} profiling \\ input \end{tabular} }                                                                                                    \\ \cline{1-3}
            \multicolumn{2}{|l|}{$\xi^{pro(fetch)}$}    & Cycles spend in function execution (data fetch) per input tuple                                                                                                                                          &                                                                                                                                       \\ \cline{1-3}
            \multicolumn{2}{|l|}{$Miss_{LLC}$}    & number of LLC miss during function execution per input tuple                                                                                                                                             &                                                                                                                                       \\ \hline
            %            \multicolumn{2}{|l|}{$\xi_{s,c}$}            & 
            %            \begin{tabular}[c]{@{}l@{}} Cycles required by $O_c$ on handling each tuple from $O_s$ \end{tabular}                                                                 
            %            & \multirow{3}{*}{
            %                \begin{tabular}[c]{@{}l@{}}profiling\\ input
            %%                    \\ 
            %%                    \\ $\xi^{pro}_{s,c}$\\ =$\xi^{fe}_{s,c}$ +$\xi^{dat}_{s,c}$ +$\xi^{com}_{s,c}$+$\xi^{mem}_{s,c}$ 
            %                    \end{tabular}
            %                } \\ \cline{1-3}
            %%            \multirow{4}{*}{}        & $\xi^{fe}_{s,c}$       
            %%            & \begin{tabular}[c]{@{}l@{}}Cycles to obtain the reference of tuple per input tuple  \end{tabular}                                                                           &                                                                                                                     \\ \cline{2-3}
            %%            & $\xi^{dat}_{s,c}$       & \begin{tabular}[c]{@{}l@{}}Cycles to fetch input data \end{tabular}                                                                            &                                                                                                                                       \\ \cline{2-3}
            %            & $\xi^{com}_{s,c}$       & \begin{tabular}[c]{@{}l@{}}Cycles spent in in-core  execution per input tuple\end{tabular}                                                                           &                                                                                                                                       \\ \cline{2-3}
            %            & $\xi^{mem}_{s,c}$       & \begin{tabular}[c]{@{}l@{}}Cycles spent in out-of-core  execution per input tuple\end{tabular}                                                                           &                                                                                                                                       \\ \hline
            %            \multicolumn{2}{|l|}{$p_{i,j}$}               & $p_{i,j}=1$ if and only if $O_j$ is allocated into $S_i$                                                                                                                        &                                                                                                                                       \\ \hline
            
            \multicolumn{2}{|l|}{$|O_j|$}                  & parallelism of each operator                                                                                                                               & \multirow{2}{*}{    \begin{tabular}[c]{@{}l@{}} optimizer \\ input \end{tabular} }                                                                                                    \\ \cline{1-3}
            \multicolumn{2}{|l|}{$L_j$, $j \in 1...m$}    & location of each operator                                                                                                                                         &                                                                                                                                       \\ \hline
            %            \multicolumn{2}{|l|}{$b$}    & batch size                                                                                                                                               &                                                                                                                                       \\ \hline
            %            \multicolumn{2}{|l|}{}
            %            \\ \hline        
%            \multicolumn{2}{|l|}{$\xi^{fetch}_{s,c}$}                        & \begin{tabular}[c]{@{}l@{}}Cycle required to fetch each input tuple from $O_s$ \end{tabular}                                                                                            &                                                                              \\ \cline{1-3}
            %            \multirow{4}{*}{}        & $\varrho^{fe}_{s,c}$                  & load reference of input tuple                                                                                                                                                                                &                                                                                                                                       \\ \cline{2-3}
            %            & $\varrho^{dat}_{s,c}$                   & Cycle required in fetch input data in a unit of time                                                                             &                                                                                                                                       \\ \cline{2-3}
            %            & $\varrho^{com}_{s,c}$                  &  Cycle required in in-core execution in a unit of time                                                                                                                       &                                                                                                                                       \\ \cline{2-3}                                                                                                                                     \\ \cline{1-3}    
            \multicolumn{2}{|l|}{$\xi_{s,c}$}                  & \begin{tabular}[c]{@{}l@{}}Total cycle required for handling each input tuples  from $O_s$               \end{tabular}                                                                                                                                                         & \multirow{1}{*}{
                \begin{tabular}[c]{@{}l@{}}\\ model \\ output
                    %                    \\ \\ $\varrho_{s,c}$\\ =$\varrho^{fe}_{s,c}$ +$\varrho^{dat}_{s,c}$ +$\varrho^{com}_{s,c}$+$\varrho^{mem}_{s,c}$
                \end{tabular}}                                                                                                         \\ \cline{1-3}
                \multicolumn{2}{|l|}{$\lambda_{s,c}$}               & 
                %            Input rate of $O_c$ from $O_s$, $\lambda_{s,c}=r_{s}$ since no lost in transmission                                                                                                                                                          &     \\ \cline{1-3}
                \begin{tabular}[c]{@{}l@{}} Input rate of $O_c$ from $O_s$
                \end{tabular}                                                                                            &                                                                              \\ \cline{1-3}
                \multicolumn{2}{|l|}{$\mu_{s,c}$}               & 
                %            processing rate of $O_c$ for handling (fetch and process) tuples from $O_s$                                                                                                  &     \\ \cline{1-3}    
                \begin{tabular}[c]{@{}l@{}} Processing rate of $O_c$ for handling tuples from $O_s$. \end{tabular}                                                                                            &                                                                              \\ \cline{1-3}            
                \multicolumn{2}{|l|}{$r_{j}$}              & Output rate of $O_j$                                                                                                &                                                                         \\ \cline{1-3}                                                
                \multicolumn{2}{|l|}{$\Psi$}                    & Estimated throughput of the stream application                                                                                                                                      &                                                                                                                                       \\ \hline
            \end{tabular}%
        }
            %\vspace{-3pt}
\end{table}
%\vspace{-3pt}

\subsection{Input Rate Estimation}
\begin{definition}
\newcompact
    \textbf{Input rate} $\lambda_{s,c}$ is defined to be the number of tuples received at operator $O_c$ in a unit of time, which are produced by operator $O_s$. 
\newcompact    
\end{definition}
Let input selectivity of $O_c$ be $\sigma^{in}$ denoting the actual portion of stream it receives from its producer $O_s$, then
\begin{align} 
     \scriptsize
    \lambda_{s,c} &= 
    \begin{cases}
    \chi\,\text{if s} \in \emptyset\\
    \sigma^{in}*r_{s}, \text{otherwise}
    \end{cases}\label{eqn:input}
\end{align}
where $r_{s}$ denotes output rate of $O_s$ and $\chi$ denotes external input stream rate of an application.
%, and is expressed in Equation~\ref{eqn:ro_c}.
    
\textbf{Parallel Operators.}
We consider each operator replica individually as an operator in our model, and we only need to extend the input estimation accordingly. In particular, $r_{s}$ is being partitioned. 

Let $p{(s,c_e)}$ denote the \textbf{partition ratio} from  $O_s$ as producer to $O_{c_e}$ as consumer. 
Then, Equation~\ref{eqn:input} shall be revised as follows,
\begin{align} 
\scriptsize
    \lambda_{s,c_e} &= 
    \begin{cases}
    \chi, \text{if s} \in \emptyset\nonumber\\
    \sigma^{in}*r_{s} * p(s,c_e), \text{otherwise} 
    \end{cases}\nonumber\\
    where\ & \sum_{e\in\ replicas\ of\ O_c} p{(s,c_e)} =1
\end{align}
    
The \textbf{total input rates} $\lambda_{c}$ denotes the total number of tuples to be received from all of the producers of $O_c$ in a unit of time, and can be hence denoted as $\sum_{s\in \vec{Prod}(c)}  \lambda_{s,c}$, where $\vec{Prod}(c)$ represents a set producers of operator $O_c$.
   
\subsection{Processing Rate Estimation}
Estimating the actual processing rate of each operator is important as it not only provides necessary information to estimate application throughput, but also the resource demands.
However, it is a challenging task due to the following reasons.
\begin{myenumerate}
    \item Due to NUMA effect, the processing rate of each operator varies depending on its placement that results in different data fetch cost. 
    \item Operator may cooperatively process tuples from different producers that correspond to different processing cost. 
    \item Input rate may or may not affect the actual processing rate depending on their relative size. 
    %\vspace{-3pt}
\end{myenumerate}

\tony{
All the above factors need to be considered for building an accurate cost model for DSP systems, which is quite different to previous studies~\cite{Viglas:2002:RQO:564691.564697}. 
In order to capture those factors, 
we first define the basic processing rate that represents the processing capability of an operator assuming it has only one producer. 
We breakdown the time of processing each tuple into two components (i.e., $\xi^{fetch}_{s,c}$ and $\xi^{pro}_{s,c}$) and take the varying remote memory access cost ($C_{RMA}$) into consideration so that the basic processing rate of an operator is aware of the relative placements.
Then, we show how to estimate total processing rate that represents the processing capability of an operator considering multiple producers. 
The total processing rate is used to estimate the cooperative processing rate that represents the processing rate of an operator to a producer when it needs to cooperatively process tuples from multiple producers.
% Finally, we estimate the actual processing rate of an operator to each of its producer when it has to cooperatively process tuples from multiple producers.
Finally, we consider both cases of over and under input supply when estimating the actual processing rate.}

\begin{definition}
\newcompact 
\textbf{Basic processing rate} $\mu_{s,c}$ is the number of tuples (from $O_s$) that can be processed by $O_c$ in a unit of time. It represents the conceptual processing capability of $O_c$ to handle tuples from $O_s$ without processing tuples from other producers.
\newcompact 
\end{definition}
Let $\xi_{s,c}$ to denote the \textbf{demand cycles per tuple} required by operator $O_c$ on handling one tuple from operator $O_s$. 
As an operator is carried by one thread, it can maximally fully occupies one CPU core. 
That is, 
\begin{align} 
\scriptsize
    \mu_{s,c}=
    \frac{\epsilon}
    {\xi^{}_{s,c}} 
    \label{eqn:process_rate_unit}
\end{align}
, where $\epsilon$ {represents the cycles available per unit of time in one CPU core.}
%$\frac{\epsilon}{\xi^{}_{s,c}}$.

We breakdown $\xi_{s,c}$ into the following non-overlapping components.
\begin{myenumerate}
\item $\xi^{fetch}_{s,c}$: Cycles required to fetch (local or remotely) the actual data of each input tuple from operator $O_s$.
\item $\xi^{pro}_{s,c}$: Cycles required in actual function execution and emitting outputs tuples per input tuple.
\end{myenumerate}

The $\xi^{pro}_{s,c}$ will not vary in different execution plans and can be obtained through profiling.
In contrast, due to NUMA, the data fetch cycles $\xi^{fetch}_{s,c}$ is determined by its relative distance to its producer, which can be represented as,
\begin{align}
 \scriptsize
    \xi^{fetch}_{s,c}&=C_{LocalAcc}+C_{RMA} + c
    \label{eqn:fecycles}
\end{align}
, where $c$ represents a constant cost mainly consists of accessing the queue data structure. It can be significantly reduced by applying local output caching (Section~\ref{sec:design}).
$C_{LocalAcc}$ refers to the cost of local data access (i.e., within the same CPU socket), and we find it is mostly severed at the last level cache (LLC). 
Therefore, $C_{LocalAcc} =\frac{|tuple|}{|cacheLine|} * {T_C}$, where $T_C$ refers to the access cost of last level cache.
On the other hand, $C_{RMA}$ refers to data transfer cost and can be estimated as $C_{RMA}= \frac{|tuple|}{|cacheLine} * \eta_{i,j} $, where $\eta_{i,j}$ represent the data transfer cost from socket $i$ (allocation of producer) to socket $j$ (allocation of consumer), which varies in different execution plans.

Let $\sigma^{br}$ be the branching ratio that determines the actual portion of input tuples being processed (otherwise being filtered), we have
\begin{align} 
\scriptsize
    \xi^{}_{s,c}&=\xi^{fetch}_{s,c}+\sigma^{br}*\xi^{pro}_{s,c}
\label{eqn:xi}
\end{align}
\begin{definition}
\newcompact 
    \textbf{Total processing rate} $\mu_{c}$ of an operator $O_c$ is defined to be the total number of tuples (from all of its producers) that can be processed in a unit of time.
\newcompact 
\end{definition}
Let's assume an arbitrary length of observation time $t$, and denote number of tuples to be processed during $t$ as $num$ and time needed to process them as $time$.
Then, we have 
\begin{align}
\scriptsize
  \mu_{c} & = \frac{num}{time},\nonumber\\
   where\ num & =\lambda_{s,c}*t, \nonumber\\
          time &=\sum_{s\in \vec{Prod(c)}}\frac{\lambda_{s,c}}{\mu_{s,c}}*t.    
\end{align}
\begin{definition}
\newcompact 
    \textbf{Cooperative processing rate} ${\widetilde{\mu}}_{s,c}$ of an operator $O_c$ is defined to be the \emph{upper bound} of the number of tuples able to be handled from $O_s$ in a unit of time in the presence of tuples from other producers.
\newcompact 
\end{definition}
As tuples from all producers are processed in a cooperative manner with equal priority~\footnote{It is possible to configure different priorities among different operators here, but is out of the scope of this paper.}, tuples will be get processed in a first come first serve manner. Therefore, given the total processing rate $\mu_{c}$, the ${\widetilde{\mu}}_{s,c}$ is proportional to the proportion of the corresponding input rate, that is,
\begin{align} 
 \scriptsize
    {\widetilde{\mu}}_{s,c}=\mu_{c}*\frac{\lambda_{s,c}}{\lambda_{c}}
\end{align}
% Clearly, ${\widetilde{\mu}}_{s,c} \leq \mu_{s,c}$, and the equality occurs when there is only one producer, i.e., $\lambda_{s,c}=\lambda_{c}$ and $\mu_{s,c}=\mu_{c}$. 

Finally, in order to estimate the \textbf{actual processing rate} of an operator ($\overline{\mu}_{s,c}$), there are two cases that we have to consider:

\begin{myenumerate}
    \item  ${\widetilde{\mu}}_{s,c}$ is large enough such that it can finish processing all its given inputs even with the need of cooperatively processing tuples from other producers. 
    In other words, it is under-supplied, and its processing rate is limited by its input rates. In this case, $\overline{\mu}_{s,c}= \lambda_{s,c}$.
    \item On the other hand, it may be over-supplied, and the expected rate is simply the cooperative processing rate, and $\overline{\mu}_{s,c}= {\widetilde{\mu}}_{s,c}$.
    %\vspace{-5pt}
\end{myenumerate}

Therefore, $\overline{\mu}_{s,c}=min({\widetilde{\mu}}_{s,c},\lambda_{s,c}).$
%\label{eqn:process_rate_expect}

\subsection{Output Rate Estimation}
%\vspace{-5pt}
\begin{definition}
\newcompact 
\textbf{Output rate} $r_{s,c}$ of an operator $O_c$ is defined to be the expected number of tuples produced in a unit of time in handling tuples from $O_s$. 
\newcompact 
\end{definition}
Let the selectivity of $O_c$ be $\sigma^{out}$, then $r_{s,c}=\overline{\mu}_{s,c}*\sigma^{out}$, and the \textbf{total output rate} $r_{c}$ can be hence expressed as $r_{c}=\sum_{s\in \vec{Prod(c)}}r_{s,c}.$

\begin{example}
\label{example}
Consider a simple application with three operators A, A' (replica of A) and B as shown in Figure~\ref{fig:estimate_example} as an example, and we are to estimate the output rate of B. 
Assume under such an execution plan that we have $\lambda_{a,b}=15$ and $\lambda_{a',b}=10$. 
Further, we are given the processing rate as $\mu_{a,b}=10$ and $\mu_{a',b}=15$ (e.g., B is collocated with A' but remotely allocated to A), respectively. 
The total processing rate $\mu_{b}$ can be estimated as,
$\mu_{b}=\frac{\lambda_{a,b}+\lambda_{a',b}}{\frac{\lambda_{a,b}}{\mu_{a',b}}+\frac{\lambda_{a,b}}{\mu_{a',b}}}=11.5.$ 
The cooperative processing rate is therefore,
${\widetilde{\mu}}_{a,b}=\mu_{b}*\frac{\lambda_{a,b}}{\lambda_{a,b}+\lambda_{a',b}}=6.9,$ and
${\widetilde{\mu}}_{a',b}=\mu_{b}*\frac{\lambda_{a',b}}{\lambda_{a,b}+\lambda_{a',b}}=4.6.$

As ${\widetilde{\mu}}_{a,b}<\lambda_{a,b}$ and ${\widetilde{\mu}}_{a',b}<\lambda_{a',b}$, the expected processing rates are both bounded by cooperative processing rates, and the aggregated output is therefore the sum of cooperative processing rate (i.e., 11.5).
\end{example}

\begin{figure}[h]
    \centering
    \includegraphics*[width=0.28\textwidth]{example}
    %\vspace{-5pt}
    \caption{Example of estimating output rate.}                   
    \label{fig:estimate_example}
\end{figure}

% \textbf{Processing rate shifting.}
We make from this example two observations. 
First, operator may experience different processing rate 
to different producers due to different relative allocations.
Second, total processing rate shifts close to the processing rate of the corresponding producer who offers relatively large input rates, i.e., operator needs to process more tuples from that producer.
%We will verify this effect in our experiments later.

==> more_results.tex <==
\section{More Experiment Settings}


==> optimization.tex <==
\section{Execution Plan Optimization}
fdfd

